Listening to the Voices: Describing Ethical Caveats of Conversational User Interfaces According to Experts and Frequent Users

Advances in natural language processing and understanding have led to a rapid growth in the popularity of conversational user interfaces (CUIs). While CUIs introduce novel benefits, they also yield risks that may exploit people's trust. Although research looking at unethical design deployed through graphical user interfaces (GUIs) established a thorough understanding of so-called dark patterns, there is a need to continue this discourse within the CUI community to understand potentially problematic interactions. Addressing this gap, we interviewed 27 participants from three cohorts: researchers, practitioners, and frequent users of CUIs. Applying thematic analysis, we construct five themes reflecting each cohort's insights about ethical design challenges and introduce the CUI Expectation Cycle, bridging system capabilities and user expectations while considering each theme's ethical caveats. This research aims to inform future development of CUIs to consider ethical constraints while adopting a human-centred approach.

==> Tables/themes-descriptions.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{0.02\linewidth}
\begin{tabular}{p{0.2\linewidth}p{0.7\linewidth}}
\hline
\textbf{Theme} & \textbf{Ethical Caveat} \\ \hline

\rowcolor[HTML]{EFEFEF} 
Building Trust and Guarding Privacy & Users feel vulnerable to use CUIs, posing a need for CUI developers to prioritise transparency and control over data handling.\\ 

Guiding Through Interactions & Guidelines and frameworks need to educate developers to develop accessible CUIs that empower users with diverse technological literacy to confidently interact with available features. \\

\rowcolor[HTML]{EFEFEF} 
Human-like Harmony & Anthropomorphic features should be implemented with care and in line with a CUI's capabilities to support intuitive and authentic interactions, preventing unrealistic expectations. \\

Inclusivity and Diversity & The development and design of CUI interactions need to consider individual needs and characteristics of users, especially marginalised groups, ensuring equitable CUI interactions. \\

\rowcolor[HTML]{EFEFEF} 
Setting Expectations & CUI capabilities should avoid deceptive interactions and, instead, be transparent to users to prevent frustration and mistrust. \\



\hline
\end{tabular}
\caption{This table summarises the five emerging themes.}
\label{tab:theme-descriptions}
\end{table}
